Data-driven prediction and control of extreme events in a chaotic flow

An extreme event is a sudden and violent change in the state of a nonlinear system. In fluid dynamics, extreme events can have adverse effects on the system's optimal design and operability, which calls for accurate methods for their prediction and control. In this paper, we propose a data-driven methodology for the prediction and control of extreme events in a chaotic shear flow. The approach is based on echo state networks, which are a type of reservoir computing that learn temporal correlations within a time-dependent dataset. The objective is five-fold. First, we exploit ad-hoc metrics from binary classification to analyse (i) how many of the extreme events predicted by the network actually occur in the test set (precision), and (ii) how many extreme events are missed by the network (recall). We apply a principled strategy for optimal hyperparameter selection, which is key to the networks' performance. Second, we focus on the time-accurate prediction of extreme events. We show that echo state networks are able to predict extreme events well beyond the predictability time, i.e., up to more than five Lyapunov times. Third, we focus on the long-term prediction of extreme events from a statistical point of view. By training the networks with datasets that contain non-converged statistics, we show that the networks are able to learn and extrapolate the flow's long-term statistics. In other words, the networks are able to extrapolate in time from relatively short time series. Fourth, we design a simple and effective control strategy to prevent extreme events from occurring. The control strategy decreases the occurrence of extreme events up to one order of magnitude with respect to the uncontrolled system. Finally, we analyse the robustness of the results for a range of Reynolds numbers. We show that the networks perform well across a wide range of regimes.

==> supp_mat.tex <==

% \unappendix
\setcounter{page}{1}
\setcounter{figure}{0}
\setcounter{section}{18}% Equivalent to "letter O"
\renewcommand{\thesection}{\Alph{section}}%
\section{supplementary material}
\subsection{Block Diagrams}

In this section, we show mathematically detailed block diagrams versions of the block diagrams reported in the main text.  

\begin{figure}[H]
\centering
\includegraphics[width=.9\textwidth]{Figures/supp_pdfresizer.com-pdf-crop.pdf}
\caption{Schematic representation of the prediction of extreme events with echo state networks. For a starting point, $t_0$, we evaluate whether the predicted kinetic energy, $k_{\mathrm{ESN}}$, and the true kinetic energy, $k_{\mathrm{True}}$, cross the extreme event threshold, $k_e$, in the interval $[t_0+\mathrm{PT},t_0+\mathrm{PT} + 1\mathrm{LT}]$, where PT is the prediction time.}
\label{fig:pr_scheme_supp}
\end{figure}

\begin{figure}[H]
\centering
\includegraphics[width=.9\textwidth]{Figures/supp_PHEE_chart.pdf}
\caption{Schematic representation of the computation of the prediction horizon for extreme events, $\mathrm{PH}_{\mathrm{ee}}$. For the $i-$th event, we evaluate if the prediction horizon \eqref{eq:PH} of the closed-loop prediction starting from $\tau_e$ before the event is larger than $\tau_e$, which is initialized  to 10LTs. If the prediction horizon is larger, $\mathrm{PH}_{\mathrm{ee}}=\tau_e$ and we analyze the next event, if not, we decrease $\tau_e$ by 0.5LTs and evaluate the prediction horizon starting from the new $\tau_e$ before the event.}
\label{fig:phee_scheme_supp}
\end{figure}

\begin{figure}[H]
\centering
\includegraphics[width=.9\textwidth]{Figures/supp_Control_Chart.pdf}
\caption{Schematic representation of the control strategy. If the ESN closed-loop starting at $t_0$ predicts an event in the interval $t_0+[\mathrm{PT},\mathrm{PT}+1\mathrm{LTs}]$, we increase the Reynolds number to 2000 from $t_0+\mathrm{PT}-1\mathrm{LTs}$ to $t_0+\mathrm{PT}+0.5\mathrm{LTs}$. The next closed-loop prediction then starts after the control strategy ends at the updated $t_0=t_0+\mathrm{PT}+0.5\mathrm{LTs}$.}
\label{fig:control_scheme_supp}
\end{figure}

\subsection{Reduced-order model}
\label{sec:reduced}

The nine modes of the MFE model \cite{moehlis2004low} described in section \ref{sec:MFE} are:

\begin{enumerate}
\item The basic profile:
\begin{equation}
\mathbf{\hat{v}_1} = \left( \begin{array}{c} \sqrt{2}\sin(\pi y/2)\\0\\0
\end{array} \right)
\end{equation}
\item The streak:
\begin{equation}
\mathbf{\hat{v}_2} = \left( \begin{array}{c}
\frac{4}{\sqrt{3}} \cos^2(\pi y/2) \cos(\gamma z)\\
0\\
0
\end{array} \right)
\end{equation}
\item The downstream vortex:
\begin{equation}
\mathbf{\hat{v}_3} = \frac{2}{\sqrt{4\gamma^2 + \pi^2}} \left( \begin{array}{c}
0\\
2\gamma \cos(\pi y/2) \cos(\gamma z)\\
\pi \sin(\pi y/2) \sin(\gamma z)
\end{array} \right)
\end{equation}
\item The spanwise flows:
\begin{equation}
\mathbf{\hat{v}_4} = \left( \begin{array}{c}
0\\
0\\
\frac{4}{\sqrt{3}} \cos(\alpha x) \cos^2(\pi y/2)
\end{array} \right)
\end{equation}
\begin{equation}
\mathbf{\hat{v}_5} = \left( \begin{array}{c}
0\\
0\\
2 \sin(\alpha x) \sin(\pi y/2)
\end{array} \right)
\end{equation}
\item The normal vortex modes:
\begin{equation}
\mathbf{\hat{v}_6} = \frac{4\sqrt{2}}{\sqrt{3(\alpha^2+\gamma^2)}}
\left( \begin{array}{c}
-\gamma\cos(\alpha x) \cos^2(\pi y/2) \sin(\gamma z) \\
0\\
\alpha \sin(\alpha x) \cos^2(\pi y/2) \cos(\gamma z)
\end{array} \right)
\end{equation}
\begin{equation}
\mathbf{\hat{v}_7} = \frac{2\sqrt{2}}{\sqrt{\alpha^2+\gamma^2}}
\left( \begin{array}{c}
\gamma\sin(\alpha x) \sin(\pi y/2) \sin(\gamma z) \\
0\\
\alpha \cos(\alpha x) \sin(\pi y/2) \cos(\gamma z)
\end{array} \right)
\end{equation}
\item A three-dimensional mode:
\begin{equation}
\mathbf{\hat{v}_8} = N_8
\left( \begin{array}{c}
\pi \alpha \sin(\alpha x) \sin(\pi y/2) \sin(\gamma z)\\
2(\alpha^2+\gamma^2) \cos(\alpha x) \cos(\pi y/2) \sin(\gamma z)\\
-\pi \gamma \cos(\alpha x) \sin(\pi y/2) \cos(\gamma z)
\end{array} \right)
\end{equation}
with 
\begin{equation}
N_8 = \frac{2\sqrt{2}}{\sqrt{(\alpha^2 + \gamma^2)(4\alpha^2 + 4\gamma^2 + \pi^2)}}
\end{equation}
\item The modification of the basic profile mode:
\begin{equation}
\mathbf{\hat{v}_9} = \left( \begin{array}{c}
\sqrt{2}\sin(3\pi y/2)\\
0\\
0
\end{array} \right)
\end{equation}

\end{enumerate}

The governing equations for the modes are:

\begin{equation}
\frac{da_1}{dt} = \frac{\beta^2}{Re} - \frac{\beta^2}{Re}a_1 - \sqrt{\frac{3}{2}} \frac{\beta \gamma}{\kappa_{\alpha \beta \gamma}}a_6 a_8 + \sqrt{\frac{3}{2}} \frac{\beta \gamma}{\kappa_{\beta \gamma}}a_2 a_3
\end{equation}
\begin{align}
\frac{da_2}{dt} = -\left( \frac{4\beta^2}{3} + \gamma^2 \right) \frac{a_2}{Re} + \frac{5\sqrt{2}}{3\sqrt{3}} \frac{\gamma^2}{\kappa_{\alpha \gamma}} a_4 a_6 - \frac{\gamma^2}{\sqrt{6} \kappa_{\alpha \gamma}} a_5 a_7 \nonumber \\
		-\frac{\alpha \beta \gamma}{\sqrt{6} \kappa_{\alpha \gamma} \kappa_{\alpha \beta \gamma}} a_5 a_8 - \sqrt{\frac{3}{2}} \frac{\beta \gamma}{\kappa_{\beta \gamma}} a_1 a_3 - \sqrt{\frac{3}{2}} \frac{\beta \gamma}{\kappa_{\beta \gamma}} a_3 a_9
\end{align}

\begin{align}
\frac{da_3}{dt} = - \frac{\beta^2 + \gamma^2}{Re} a_3 + \frac{2}{\sqrt{6}} \frac{\alpha \beta \gamma}{\kappa_{\alpha \gamma} \kappa_{\beta \gamma}}(a_4 a_7 + a_5 a_6) + \frac{\beta^2(3\alpha^2 + \gamma^2) - 3\gamma^2 (\alpha^2 + \gamma^2)}{\sqrt{6} \kappa_{\alpha\gamma} \kappa_{\beta \gamma} \kappa_{\alpha \beta \gamma}} a_4 a_8
\end{align}
\begin{align}
\frac{da_4}{dt} = & - \frac{3\alpha^2 + 4\beta^2}{3 Re} a_4 - \frac{\alpha}{\sqrt{6}} a_1 a_5 - \frac{10}{3\sqrt{6}} \frac{\alpha^2}{\kappa_{\alpha\gamma}} a_2 a_6 \nonumber \\
	&- \sqrt{\frac{3}{2}} \frac{\alpha \beta \gamma}{\kappa_{\alpha\gamma}\kappa_{\beta\gamma}} a_3 a_7 - \sqrt{\frac{3}{2}} \frac{\alpha^2 \beta^2}{\kappa_{\alpha\gamma}\kappa_{\beta\gamma}\kappa_{\alpha\beta\gamma}}a_3 a_8 - \frac{\alpha}{\sqrt{6}}a_5 a_9
\end{align}
\begin{align}
\frac{da_5}{dt} = - \frac{\alpha^2 + \beta^2}{Re}a_5 + \frac{\alpha}{\sqrt{6}} a_1 a_4 + \frac{\alpha^2}{\sqrt{6}} a_1 a_4 + \frac{\alpha^2}{\sqrt{6}\kappa_{\alpha\gamma}}a_2 a_7 \nonumber \\
	- \frac{\alpha \beta \gamma}{\sqrt{6} \kappa_{\alpha \gamma}\kappa_{\alpha\beta\gamma}}a_2 a_8 + \frac{\alpha}{\sqrt{6}} a_4 a_9 + \frac{2}{\sqrt{6}} \frac{\alpha \beta \gamma}{\kappa_{\alpha\gamma}\kappa_{\beta\gamma}} a_3 a_6
\end{align}
\begin{align}
\frac{da_6}{dt} =& - \frac{3\alpha^2 + 4\beta^2 + 3\gamma^2}{3Re}a_6 + \frac{\alpha}{\sqrt{6}} a_1 a_7 + \sqrt{\frac{3}{2}} \frac{\beta \gamma}{\kappa_{\alpha\beta\gamma}} a_1 a_8 \nonumber \\
	&+ \frac{10}{3\sqrt{6}} \frac{\alpha^2 - \gamma^2}{\kappa_{\alpha\gamma}} a_2 a_4 - 2\sqrt{\frac{2}{3}} \frac{\alpha\beta\gamma}{\kappa_{\alpha\gamma}\kappa_{\beta\gamma}}a_3 a_5 + \frac{\alpha}{\sqrt{6}}a_7a_9 + \sqrt{\frac{3}{2}} \frac{\beta \gamma}{\kappa_{\alpha\beta\gamma}}a_8a_9
\end{align}
\begin{align}
\frac{da_7}{dt} = -\frac{\alpha^2 + \beta^2 + \gamma^2}{Re} a_7 - \frac{\alpha}{\sqrt{6}} (a_1 a_6 + a_6 a_9) + \frac{1}{\sqrt{6}} \frac{\gamma^2 - \alpha^2}{\kappa_{\alpha\gamma}} a_2 a_5 + \frac{1}{\sqrt{6}} \frac{\alpha \beta \gamma}{\kappa_{\alpha\gamma}\kappa{\beta\gamma}}a_3a_4
\end{align}
\begin{align}
\frac{da_8}{dt} =  -\frac{\alpha^2 + \beta^2 + \gamma^2}{Re} a_8 + \frac{2}{\sqrt{6}} \frac{\alpha \beta \gamma}{\kappa_{\alpha\gamma}\kappa_{\alpha\beta\gamma}}a_2a_5 + \frac{\gamma^2(3\alpha^2-\beta^2+3\gamma^2)}{\sqrt{6}\kappa_{\alpha\gamma}\kappa_{\beta\gamma}\kappa_{\alpha\beta\gamma}}a_3a_4
\end{align}
\begin{align}
\frac{da_9}{dt} = -\frac{9\beta^2}{Re}a_9 + \sqrt{\frac{3}{2}} \frac{\beta\gamma}{\kappa_{\beta\gamma}}a_2a_3 - \sqrt{\frac{3}{2}} \frac{\beta\gamma}{\kappa_{\alpha\beta\gamma}} a_6a_8
\end{align}
where
\begin{gather}
\kappa_{\alpha\gamma} = \sqrt{\alpha^2+\gamma^2}, \quad
\kappa_{\beta\gamma} = \sqrt{\beta^2+\gamma^2}, \quad
\kappa_{\alpha\beta\gamma} = \sqrt{\alpha^2+\beta^2+\gamma^2} \nonumber \\
\nonumber \\
\alpha = \frac{2\pi}{L_x}, \quad
\beta = \frac{\pi}{2}, \quad
\gamma = \frac{2\pi}{L_z}.
\end{gather}


